MarkLLM: An Open-Source Toolkit for LLM Watermarking

LLM watermarking, which embeds imperceptible yet algorithmically detectable signals in model outputs to identify LLM-generated text, has become crucial in mitigating the potential misuse of large language models. However, the abundance of LLM watermarking algorithms, their intricate mechanisms, and the complex evaluation procedures and perspectives pose challenges for researchers and the community to easily experiment with, understand, and assess the latest advancements. To address these issues, we introduce MarkLLM, an open-source toolkit for LLM watermarking. MarkLLM offers a unified and extensible framework for implementing LLM watermarking algorithms, while providing user-friendly interfaces to ensure ease of access. Furthermore, it enhances understanding by supporting automatic visualization of the underlying mechanisms of these algorithms. For evaluation, MarkLLM offers a comprehensive suite of 12 tools spanning three perspectives, along with two types of automated evaluation pipelines. Through MarkLLM, we aim to support researchers while improving the comprehension and involvement of the general public in LLM watermarking technology, fostering consensus and driving further advancements in research and application. Our code is available at https://github.com/THU-BPM/MarkLLM.

==> tables/algs.tex <==
\begin{table*}[h!]
\caption{Details of watermarking algorithms supported in MarkLLM.}
\centering
\begin{tabular}{p{5cm} p{3cm} p{7cm}}
\hline
\small Algorithm Name & \small Category & \small Methodology \\ \hline
\small KGW \citep{DBLP:conf/icml/KirchenbauerGWK23} & \small KGW Family & \small Separate the vocabulary set into two lists: a red list and a green list based on the preceding token, then add bias to green tokens so that the LLM-produced text exhibits preference of using green tokens.\\ 
\small Unigram \citep{zhao2023provable} & \small KGW Family & \small Use a globally fixed red-green list separation for every location, aiming to enhance robustness against tampering. \\ 
\small SWEET \citep{lee2023wrote} & \small KGW Family & \small Modifications to the logits are selectively applied only to high-entropy locations while bypassing low-entropy ones, aiming to improve text quality in low-entropy scenarios, such as code generation. \\ 
\small UPV \citep{liu2024an} & \small KGW Family & \small Train one network as a generator for segregating red-green lists and another network as a detector for directly providing a classification result based on textual input. The distinction between the generator network and the detector network enables public detection.\\ 
\small EWD \citep{lu2024entropy} & \small KGW Family & \small During the watermark detection phase, each token is assigned a different weight based on its entropy, with tokens having higher entropy receiving greater weight. This approach aims to enhance watermark detectability in low-entropy situations.\\
\small SIR \citep{liu2024a} & \small KGW Family & \small Train a generator network to convert token embeddings into context-aware biases, thereby enhancing robustness against semantic invariant tampering. \\ 
\small X-SIR \citep{he2024can} & \small KGW Family & \small The red-green partition of the vocabulary no longer operates at the token level but rather at the level of semantic clusters, grouping semantically similar words together within the same group and adding bias at the group level. This shift from adding bias to individual green tokens to green clusters is designed to enhance robustness against Cross-lingual Watermark Removal Attacks (CWRA). \\ 
\small EXP \citep{aronsonpowerpoint} & \small Christ Family & \small Utilize a pseudo-random sequence based on preceding tokens to guide token sampling when generating each new token through the exponential (EXP) sampling rule. As a result, the watermarked text displays a degree of alignment with the sequence, aiding in its detection. \\ 
\small EXP-Edit \citep{kuditipudi2023robust} & \small Christ Family & \small Expanding on the use of the EXP sampling rule, introduce the concept of edit distance to measure the alignment between the pseudo-random sequence and the text, which significantly improves its robustness against tampering.\\ \hline
\end{tabular}
\label{tab:supported_algorithms}
\end{table*}

==> tables/detectability.tex <==
\begin{table*}[h!]
\caption{
The evaluation results of assessing the detectability of nine algorithms supported in MarkLLM. 200 watermarked texts are generated, while 200 non-watermarked texts serve as negative examples. We furnish TPR and F1-score under dynamic threshold adjustments for 10\% and 1\% FPR, alongside TPR, TNR, FPR, FNR, P, R, F1, ACC at optimal performance.
}
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{lcc|cc|cccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{10\%FPR} & \multicolumn{2}{c}{1\%FPR} & \multicolumn{8}{c}{Best}\\
\cmidrule(r){2-13}
    & TPR & F1 & TPR & F1 & TPR & TNR & FPR & FNR & P & R & F1 & ACC \\
\midrule
KGW & \textbf{1.000} & \textbf{0.955} & 0.995 & 0.993 & \textbf{1.000} & 0.995 & 0.005 & \textbf{0.000} & 0.995 & \textbf{1.000} & 0.998 & 0.998 \\
Unigram & \textbf{1.000} & 0.950 & \textbf{1.000} & 0.993 & \textbf{1.000} & \textbf{1.000} & \textbf{0.000} & \textbf{0.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
SWEET & \textbf{1.000} & 0.952 & \textbf{1.000} & \textbf{0.995} & \textbf{1.000} & \textbf{1.000} & \textbf{0.000} & \textbf{0.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
UPV & $\times$ & $\times$ & $\times$ & $\times$ & \textbf{1.000} & 0.990 & 0.010 & \textbf{0.000} & 0.990 & \textbf{1.000} & 0.995 & 0.995 \\
EWD & \textbf{1.000} & 0.952 & \textbf{1.000} & \textbf{0.995} & \textbf{1.000} & \textbf{1.000} & \textbf{0.000} & \textbf{0.000} & \textbf{1.000}& \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
SIR & \textbf{1.000} & 0.952 & 0.990 & 0.990 & 0.985 & \textbf{1.000} & \textbf{0.000} & 0.015 & \textbf{1.000} & 0.985 & 0.992 & 0.993 \\
X-SIR & 0.990 & 0.947 & 0.935 & 0.961 & 0.985 & 0.980 & 0.020 & 0.015 & 0.980 & 0.985 & 0.983 & 0.983 \\
EXP & \textbf{1.000} & 0.952 & \textbf{1.000} & \textbf{0.995} & \textbf{1.000} & \textbf{1.000} & \textbf{0.000} & \textbf{0.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\
EXP-Edit & \textbf{1.000} & 0.952 & 0.995 & 0.990 & 0.995 & 0.985 & 0.015 & 0.005 & 0.985 & 0.995 & 0.990 & 0.990 \\
\bottomrule
\end{tabular}
}
\vspace{1em}

\label{tab:detectability}
\end{table*}



==> tables/quality.tex <==
\begin{table*}[h!]
\caption{
The evaluation results of assessing the text quality impact of the nine algorithms supported in MarkLLM. We compared 200 watermarked texts with 200 non-watermarked texts. However, due to dataset constraints, only 100 watermarked texts were compared with 100 non-watermarked texts for code generation.
}
\vspace{10pt}
\centering
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{lcc|cc|c}
\toprule
\multirow{3}{*}{Method} & \multicolumn{2}{c}{Direct Analysis} & \multicolumn{2}{c}{Referenced Analysis} & External Discriminator \\
\cmidrule(r){2-6}
& \multirow{2}{*}{PPL(Ori.= 7.670)} & \multirow{2}{*}{Log Diversity(Ori.= 8.517)} & Machine Translation & Code Generation & Machine Translation\\
& & & BLEU(Ori.=31.807) & pass@1(Ori.= 43.0) & GPT-4 Judge (Wat. Win Rate)\\
\midrule
KGW & 13.776 $\uparrow$ & 7.989 $\downarrow$  & 28.242 $\downarrow$ & 34.0 $\downarrow$ & 0.31 \\
Unigram & 14.180 $\uparrow$ & 7.242 $\downarrow$ & 26.075 $\downarrow$ & 32.0 $\downarrow$ & \textbf{0.33} \\
SWEET & 12.653 $\uparrow$ & 8.086 $\downarrow$ & 28.242 $\downarrow$ & \textbf{37.0} $\downarrow$ & 0.31 \\
UPV & 11.270 $\uparrow$ & 7.698 $\downarrow$ & 28.270 $\downarrow$ & \textbf{37.0} $\downarrow$ & 0.31 \\
EWD & 13.802 $\uparrow$ & 8.220 $\downarrow$ & 28.242 $\downarrow$ & 34.0 $\downarrow$ & 0.30\\
SIR & 14.692 $\uparrow$ & 7.990 $\downarrow$ & \textbf{28.830} $\downarrow$ & \textbf{37.0} $\downarrow$ & 0.31 \\
X-SIR & 12.418 $\uparrow$ & 7.930 $\downarrow$ & 28.161 $\downarrow$ & 36.0 $\downarrow$ & \textbf{0.33} \\
EXP & \textbf{9.597} $\uparrow$ & 8.187 $\downarrow$ & $\times$ & 20.0 $\downarrow$ & $\times$ \\
EXP-Edit & 11.490 $\uparrow$ & \textbf{9.046} $\uparrow$ & $\times$ & 14.0 $\downarrow$ & $\times$\\

\bottomrule
\end{tabular}
}
\vspace{1em}

\label{tab:quality}
\end{table*}

==> tables/robustness.tex <==
\begin{table*}[h!]
\caption{
The evaluation results of assessing the robustness of nine algorithms supported in MarkLLM. For each attack, 200 watermarked texts are generated and subsequently tampered, with an additional 200 non-watermarked texts serving as negative examples. We report the TPR and F1-score at optimal performance under each circumstance.
}
\vspace{10pt}
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{lcc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{No Attack} & \multicolumn{2}{c}{Word-D} & \multicolumn{2}{c}{Word-S} & \multicolumn{2}{c}{Word-S (Context)} & \multicolumn{2}{c}{Doc-P (GPT-3.5)} & \multicolumn{2}{c}{Doc-P (Dipper)} \\
\cmidrule(r){2-13}
& TPR & F1 & TPR & F1 & TPR & F1 & TPR & F1 & TPR & F1 & TPR & F1 \\
\midrule
KGW & \textbf{1.000} & 0.998 & 0.990 & 0.982 & 0.965 & 0.967 & \textbf{1.000} & 0.990 & 0.845 & 0.858 & 0.880 & 0.878 \\
Unigram & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.995 & \textbf{0.995} & \textbf{1.000} & \textbf{1.000} & \textbf{0.975} & \textbf{0.958} & \textbf{0.955} & \textbf{0.962} \\
SWEET & \textbf{1.000} & \textbf{1.000} & 0.985 & 0.990 & 0.945 & 0.950 & 0.995 & 0.995 & 0.870 & 0.868 & 0.840 & 0.875 \\
UPV & \textbf{1.000} & 0.995 & 0.970 & 0.980 & 0.885 & 0.896 & 0.985 & 0.961 & 0.925 & 0.906 & 0.862 & 0.864 \\
EWD & \textbf{1.000} & \textbf{1.000} & 0.990 & 0.995 & 0.940 & 0.933 & 0.995 & 0.985 & 0.880 & 0.850 & 0.930 & 0.893 \\
SIR & 0.985 & 0.992 & 0.995 & 0.997 & 0.932 & 0.956 & 0.940 & 0.970 & 0.880 & 0.910 & 0.930 & 0.896 \\
X-SIR & 0.985 & 0.983 & 0.975 & 0.977 & 0.900 & 0.890 & 0.920 & 0.934 & 0.860 & 0.823 & 0.860 & 0.835 \\
EXP & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} & 0.995 & 0.930 & 0.928 & 0.975 & 0.973 & 0.720 & 0.776 & 0.800 & 0.812 \\
EXP-Edit & 0.995 & 0.990 & \textbf{1.000} & 0.993 & \textbf{1.000} & 0.988 & \textbf{1.000} & 0.988 & 0.890 & 0.927 & 0.862 & 0.881 \\

\bottomrule
\end{tabular}
}
\vspace{1em}

\label{tab:robustness}
\end{table*}

==> tables/tools_parameters.tex <==
\begin{table}[h!]
    \caption{Hyperparamers of evaluation tools used in experiment.}
    \centering
    \begin{tabular}{ll}
    \hline
        \small Tools & \small Hyperparameters \\ \hline
        \small FundamentalSuccessRateCalculator & \small None \\
        \small DynamicThresholdSuccessRateCalculator & \small None \\
        \small WordDeletion & \small ratio: 0.3 \\ 
        \small SynonymSubstitution & \small ratio: 0.5 \\ 
        \small ContextAwareSynonymSubstitution & \small ratio: 0.5 \\ 
        \small GPTParaphraser & \small openai\_model: "gpt-3.5-turbo",  prompt: "Please rewrite the following text: " \\
        \small DipperParaphraser & \small lex\_diversity: 60, order\_diversity: 0, max\_new\_tokens: 100, do\_sample: True, top\_p: 0.75 \\ 
        \small PPLCalculator & \small model: Llama-2-13B, tokenizer: Llama-2-13B \\
        \small LogDiversityAnalyzer & \small None \\
        \small BLEUCalculator & \small None \\
        \small PassOrNotJudger & \small None \\
        \small GPTTextDiscriminator & \small openai\_model: "gpt-4", task\_description: “Translate the following German text to English.” \\\hline
        
    \end{tabular}
    \label{tab:tools_parameters}
\end{table}
